Multi-Broadcasting under the SINR Model

We study the multi-broadcast problem in multi-hop wireless networks under the SINR model deployed in the 2D Euclidean plane. In multi-broadcast, there are $k$ initial rumours, potentially belonging to different nodes, that must be forwarded to all $n$ nodes of the network. Furthermore, in each round a node can only transmit a small message that could contain at most one initial rumor and $O(\log n)$ control bits. In order to be successfully delivered to a node, transmissions must satisfy the (Signal-to-Inference-and-Noise-Ratio) SINR condition and have sufficiently strong signal at the receiver. We present deterministic algorithms for multi-broadcast for different settings that reflect the different types of knowledge about the topology of the network available to the nodes: (i) the whole network topology (ii) their own coordinates and coordinates of their neighbors (iii) only their own coordinates, and (iv) only their own ids and the ids of their neighbors. For the former two settings, we present solutions that are scalable with respect to the diameter of the network and the polylogarithm of the network size, i.e., $\log^c n$ for some constant $c> 0$, while the solutions for the latter two have round complexity that is superlinear in the number of nodes. The last result is of special significance, as it is the first result for the SINR model that does not require nodes to know their coordinates in the plane (a very specialized type of knowledge), but intricately exploits the understanding that nodes are implanted in the 2D Euclidean plane.

==> results-lower.tex <==
\subsection{Lower bound}





\begin{theorem}\label{th:lower}
For any deterministic multi-broadcast algorithm $\cA$
and for every $D\geq 3$ and $\Delta\ge 4$, there exists a network of at most $D\Delta$ nodes with diameter
$D$ and maximum node degree $\Delta$ on which algorithm $\cA$ completes broadcasting in $\Omega(D\Delta)$
rounds 
in the setting where
%
%(i) 
nodes do not know their coordinates but know ids of their neighbors. 
%or \\
%
%(ii) nodes do not know their neighbors but may know their own coordinates.
\end{theorem}


\begin{proof}
We show that the lower bound holds even for broadcasting one rumor.
We use the class of networks introduced in~\cite{JKS-ICALP-13}.
Recall that $\gamma=r/\sqrt{2}$.
%=1/\sqrt{2}$.
Consider a family of networks $\m{F}=\{F_j: 1\le j\le\Delta\}$,
each $F_j$ being of diameter $3$ and consisting of three layers:
\begin{itemize}
\vspace*{-1ex}
\item
the source $s$,
located in the origin point $(0,0)$,
is the only element of $L_1$;
\vspace*{-1ex}
\item
$L_2$ consists of $\Delta$ nodes $v_0,\ldots,v_{\Delta-1}$, where the position of $v_i$
is $(\gamma\cdot \frac{i}{\Delta}, \gamma)$ for $0\le i\le\Delta-1$;
\vspace*{-1ex}
\item
$L_3$ contains only one node $w_j$ with coordinates
$(\gamma\cdot\frac{j}{\Delta},\gamma+r)$.
%$(\frac{j}{\Delta},\gamma+1-\frac{1}{2\Delta})$.
%\tj{zmienilem wspolrzedna $w_j$ w zwiazku z $\cN$}
%for $j\in[1,\Delta]$.
\end{itemize}
Thus, the family $\m{F}$ consists of $\Delta$ elements, each network $F_j\in \m{F}$ is
uniquely determined by the
value $j$ fixing the position of node $w_j$ in $L_3$.

%In what follows, we assume that the ranges of $s$ and $v_0,\ldots,v_{\Delta-1}$ are
%equal to $r$.
%$1$.
%Then,
Observe that
\begin{itemize}
\vspace*{-1ex}
\item
$v_0,\ldots,v_{\Delta-1}$ are in the range area of $s$;
%\dk{to chyba nie zachodzi, jesli $\gamma=\sqrt{2}$,
%moze raczej powinno byc $\gamma=1/\sqrt{2}$?}
\vspace*{-1ex}
\item
$w_j$ is in the range of $v_j$ and it is not in the range of any other station from $L_1\cup L_2$;
\vspace*{-1ex}
\item
if more than $2^{\alpha/2}$ stations from $L_2$ transmit in a round, node $w_j$ cannot hear a message.
\end{itemize}
\vspace*{-1ex}
The first two bullets follow directly from the location of points.
% and the value of range.
The last bullet holds because the minimum (maximum) of the distances between $v_i$ and $w_j$ is larger
than or equal to $r$ (smaller than $r\sqrt{2}$), which guarantees that %(\ref{e:sinr})
$SINR(v_i,w_j,\m{T})$ %at node $w_j$
is smaller than $\beta=1$ for each of the transmitting stations $v_i$
if $|\m{T}\cap L_2|\geq 3$, where $\m{T}$ is the set of transmitting stations.
%Moze jednak powinny byc trzy stacje? wowczas trzeba by zmodyfikowac algorytm adversary
%dla $3$ stacji oraz $\Delta/3$, oraz potem Corollary 1 warunek na $n$.
%Chyba ze zalozymy noise $\cN=1$.}

Consider any broadcasting algorithm $\cA$. % in the uniform unknown model.
%i.e., under assumption~(a) of the Lemma.
In the beginning each node knows the set of its neighbors, i.e., nodes in range~$r$.
We specify an adversary
who simultaneously, round after round, decides
%who determines
what is heard by stations in $L_1\cup L_2$ in consecutive rounds of $\cA$
%by restricting
and restricts the family of considered networks $\m{F}$ to the networks on which
such answers are valid.
The goal of the adversary is to
prevent the arrival of a message to $w_j$ as long as possible.
Assume that the source sends the broadcast message to all nodes in $L_1$ in round $0$.
The adversary determines the family $\m{F}_t$, for every $t\leq \lfloor\Delta/2\rfloor-1$, in the following
way:
\begin{enumerate}
\vspace*{-1ex}
\item $\m{F}_0\leftarrow \m{F}$
\vspace*{-1ex}
\item $c\gets \lceil 2^{\alpha/2}\rceil$
\vspace*{-1ex}
\item For $t=1,2,\ldots, \lfloor \Delta/c\rfloor -1$ do:
 \begin{enumerate}
\vspace*{-1ex}
 \item
 if $v_{i_1}, \ldots, v_{i_{c'}}$ are the only stations from $L_1$ that transmit
 a message in the $t$-th round of $\cA$
 %(including the case when $i_1=i_2$)
 on the networks from $\m{F}_{t-1}$, and $c'\leq c$ \\
 then
 $\m{F}_t\leftarrow \m{F}_{t-1}\setminus\{F_{i_1},\ldots,F_{i_c}\}$;
%$\m{F}_t\leftarrow \m{F}_{t-1}\setminus\{F_{v_{i_1}},F_{v_{i_2}}\}$;
\vspace*{-.5ex}
 \item
 otherwise, $\m{F}_t\leftarrow \m{F}_{t-1}$.
 \end{enumerate}
\end{enumerate}
\vspace*{-1ex}
One can easily verify that, for each $t\leq \lfloor \Delta/c\rfloor -1$,
the following conditions are satisfied:
\begin{itemize}
\vspace*{-1ex}
\item
$\m{F}_t$ is not empty;
\vspace*{-1ex}
\item
the history of communication
(i.e., messages/noise heard by all stations in consecutive rounds)
is the same in each network from $\m{F}_t$ up to the round $t$;
\vspace*{-1ex}
\item
$w_j$ does not
receive the broadcast message by round $t$ in the execution of $\cA$ on any network in~$\m{F}_t$.
\end{itemize}
\vspace*{-1ex}
This provides the claimed lower bound for constant eccentricity $D$.
%under model assumption~(a).
In order to generalize this bound for arbitrary $D$, one can
consider a family of networks which consists of $(D-1)/2$ networks
from $\m{F}$
shifted
%combined
such that the source of the $i$th
network is equal to the only element in layer
$L_3$
%$L_2$
in the $(i-1)$st
network,
for $2\le i\le (D-1)/2$.
The above strategy of the adversary
can be applied sequentially to every subsequently shifted network from $\m{F}$, to gain
the multiplicative factor $D$.
Note also that the size of the obtained network is $\frac{D-1}{2}\cdot (\Delta+1)+1\le D\Delta$,
its maximum degree is $\Delta$ and its eccentricity is $\frac{D-1}{2}\cdot 2 +1=D$.
%
\end{proof}


\begin{corollary}
\label{cor:lowerGranularity}
For any deterministic broadcasting algorithm $\cA$ in
unknown uniform model,
%or known nonuniform model with two ranges,
and for any each $D\geq 3$ and $g\ge 4$, there exists a network with eccentricity
$D$ and granularity $g$ on which algorithm $\cA$ completes broadcasting in $\Omega(D g)$
rounds.
\end{corollary}
\begin{proof}
Note that granularity of the family of networks considered in the proof of
Theorem~\ref{th:lower} is $\Omega(\Delta)$, which immediately gives the claimed
result.
%\dk{tego rezultatu nie jestem pewien - dla jednej sieci ok, ale jak skladamy sieci to granularity rosnie.}
\end{proof}

==> results-section7.tex <==
\section{Networks Without Knowledge of Co-ordinates}

We consider two settings: with and without the knowledge of ids of the neighbors.
In both of them, all nodes are assumed to be awake in the beginning, i.e., we consider the spontaneous wake-up model.
[[[Does it also mean that $k=n$?]]]

\subsection{Local Knowledge Setting}

In this section we consider the setting in which every node has no knowledge of the co-ordinates of any node, but  possesses the knowledge of the labels of itself and its neighbours, as well as the values of $n$ and $N$. 
Note that a dilution cannot be directly applied in this setting, as it relies heavily on the knowledge of coordinates. 
A strong selector of appropriate size can instead be used to ensure reliable communication.

\begin{proposition}
\label{prop:no_cord_ssf}
For each $\alpha >2$, there exists a constant $d$ which depends only on model parameters, satisfying the following property. Let $W$ be a set of stations such that for each box $C$ of the grid $G_{l}$, $|W \cap C| \leq 1$; Then, the execution of any $SSF(d,N)$ ensures that the transmission of $u \in W$ is received successfully by all nodes $v$ such that $box(v) = box(u)$.
\end{proposition}


%\subsubsection{Message Dissemination}

Based on Proposition~\ref{prop:no_cord_ssf}, we simulate well-known push operation,
c.f., Algorithm~\ref{prot:no_cord_diss}. We call it {\em Coordinates-Ind-Push($v$,$S$)}.
In this procedure, a node only transmits if it is has the least label among all the active nodes in its neighbourhood. For each box $C$ of the pivotal grid, there is at most one node transmitting. Using Proposition \ref{prop:no_cord_ssf}, all transmissions are successful. This node then becomes inactive.

\alglanguage{pseudocode}
\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h]
\caption{Coordinates-Ind-Push(Node $v$, Neighbours $S$)}
\label{prot:no_cord_diss}
\begin{algorithmic}[1]
	\If{$v = \min\{S\}$}
		\State $v$ transmits its message in $SSF(c,N)$
		\Comment \emph{the first unsent message}
	\EndIf
	\State $state(v) \gets$ inactive
\Statex
\end{algorithmic}
\end{algorithm}

\begin{proposition}
\label{thm:no_cord_ssf}
Executing Algorithm~\ref{prot:no_cord_diss} $O((n+k) \log N)$ times ensures that the multicast completes successfully.
\end{proposition}

\begin{proof}

[[[I am not sure if the current algorithm works - how to recognise who is active and who isn't?
Someone might be "re-activated" after receiving a new message, and it has to transmit it as other nodes
in the box and outside may not be aware of that message]]]

\end{proof}


\subsection{No Knowledge Setting}

Now we relax the setting of the previous section and assume that each node is only aware of its label, 
apart of the usual knowledge of $n$ and $N$. 
Leaders are elected in each box of the pivotal grid in the same manner as in \emph{Gran-Dep-Collect-Info}. The leader is aware of the nodes it has \emph{defeated}, and coordinates a round robin procedure on them.

\subsubsection{Leader Election}

%Given a leader in each box of a grid $G_x$, the following two properties are maintained at every step of our protocol.
Our goal is to design a protocols guarantying the following two properties in every box of grid $G_x$:
\begin{enumerate}
\item Every node is either a leader or has been \emph{defeated} by a leader.
\item Every leader knows the messages of all the nodes it has defeated and maintains a \emph{message tree} $T$.
\end{enumerate}
[[[Definitions of "being defeated" and "message tree" are needed here]]]
The protocol, called {\em Coordinates-Ind-Leader-Election(Vertex $v$)}, is given as Algorithm~\ref{prot:no_cord_gath}.

\alglanguage{pseudocode}
\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h]
\caption{Coordinates-Ind-Leader-Election(Vertex $v$)}
\label{prot:no_cord_gath}
\begin{algorithmic}[1]
	\State $state(v)$ is active initially for all nodes.
	\For{$i = 1,2,\dots,\log g$}
		\State Each active node in $G_{2y}$ transmits its label using an $SSF(c,N)$.
		\Comment {\emph{There are only four such nodes}}
		\If{$v$ hears $m_u$}
			\If{$u < v$}
				\State $state(v) \gets inactive$
			\Else
				\State $v$ stores $m_u$
				\Comment{\emph{$v$ is the parent of $u$ in $T$}}
			\EndIf
		\EndIf
	\EndFor
\Statex
\end{algorithmic}
\end{algorithm}

\begin{lemma}
Algorithm~\ref{prot:no_cord_gath} satisfies properties 1 and 2 and completes in time
%elects at most one leader in each box of the pivotal grid such that Properties 1 and 2 are satisfied in 
$O(\log g \log N)$.
\end{lemma}

\begin{proof}

[[[Again, my biggest concern here is how to recognise who is active and who is not?
Also, the tree is a local variable. Also, what happens with the message of $v$ when it becomes inactive?]]]

\end{proof}


\subsubsection{Round Robin}

Each leader maintains the message tree $T$ of all the nodes it has defeated, which it uses to conduct a round robin in a similar manner to procedure $Thread 2$ from Section~\ref{s:only-own-coord}, c.f., Algorithm~\ref{prot:gath}. 

\alglanguage{pseudocode}
\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h]
\caption{Cord-Ind-Round-Robin(Vertex $v$)}
\label{prot:roundrobin}
\begin{algorithmic}[1]
	\State $q \gets$ empty queue
	\State $leader \gets l(G(v))$
	\State $q.$enqueue$(leader)$
	\While{not $q.$empty}
		\If{$t \mod 2 = 0$}
			\State $u \gets q.$dequeue()
			\State $leader$ transmits $m_{req}$ encoding request for $u$ to transmit its children.
			\Comment \emph{all transmissions occur through $SSF(c,N)$}
			\State $u$ transmits $\{w| w \in G(u)\}$  sequentially
			\State $u$ transmits $m_{end}$ stating it has finished transmitting its children
			\State $u$ transmits the first new message it has
			\State $q.$enqueue($u.children$)
			\Comment {\emph{as inferred from $G(u)$}}
		\EndIf
	\EndWhile
\Statex
\end{algorithmic}
\end{algorithm}

\begin{theorem}
Executing Protocol \ref{prot:no_cord_gath} followed by repeated execution of Protocol \ref{prot:roundrobin} accomplishes multi broadcasting in $O((n +\log g) \log N)$ in the setting where each node is aware only of its own label and the model parameters.
\end{theorem}

\begin{proof}

[[[First of all, in the pseudocode no original message $m_v$ is transmitted]]]

\end{proof}
